The Oddly Quiet Universe: How the CMB challenges cosmology's standard model

We discuss selected large-scale anomalies in the maps of temperature anisotropies in the cosmic microwave background. Specfically, these include alignments of the largest modes of CMB anisotropy with one another and with the geometry and direction of motion of the Solar System, and the unexpected absence of two-point angular corellations especially outside the region of the sky most contaminated by the Galaxy. We discuss these findings in relation to expectations from standard inflationary cosmology. This paper is adapted from a talk given by one of us (GDS) at the SEENET-2011 meeting in August 2011 on the Serbian bank of the Danube River.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
% that are currently in use and accepted by Romanian Journal of Physics.

%Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

%Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
\providecommand{\pd}{\ensuremath{\partial}}
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}

%bras and kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
%the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}

%Commands for multiple indexes around a central token #1
%The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
%the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
%that it diminishes the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}

%put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}

%A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

